Scope of Pre-trained Language Models for Detecting Conflicting Health Information

An increasing number of people now rely on online platforms to meet their health information needs. Thus identifying inconsistent or conflicting textual health information has become a safety-critical task. Health advice data poses a unique challenge where information that is accurate in the context of one diagnosis can be conflicting in the context of another. For example, people suffering from diabetes and hypertension often receive conflicting health advice on diet. This motivates the need for technologies which can provide contextualized, user-specific health advice. A crucial step towards contextualized advice is the ability to compare health advice statements and detect if and how they are conflicting. This is the task of health conflict detection (HCD). Given two pieces of health advice, the goal of HCD is to detect and categorize the type of conflict. It is a challenging task, as (i) automatically identifying and categorizing conflicts requires a deeper understanding of the semantics of the text, and (ii) the amount of available data is quite limited. In this study, we are the first to explore HCD in the context of pre-trained language models. We find that DeBERTa-v3 performs best with a mean F1 score of 0.68 across all experiments. We additionally investigate the challenges posed by different conflict types and how synthetic data improves a model's understanding of conflict-specific semantics. Finally, we highlight the difficulty in collecting real health conflicts and propose a human-in-the-loop synthetic data augmentation approach to expand existing HCD datasets. Our HCD training dataset is over 2x bigger than the existing HCD dataset and is made publicly available on Github.

==> Notes/plans.tex <==

\section{List of things needed: priority}
\begin{enumerate}
    \item is the abstract and intro well-written?
    % a poorly written intro / abstract is one of the most common reason to get rejection
        \item Paper title+ intro: interesting, informative?

    \item is the problem well defined? need examples of conflicts, illustrated examples of our solution
    \item are all the obvious baselines considered in the experiment section?

    \item is the exp. evaluation reasonable? convincing?
    \item does the experiment supports our claim? make sure we avoid underselling and overclaiming
    \item implications of the results: 
    
   
   
\end{enumerate}


\section{List of things needed: things that don't make our paper but can break it}
\begin{enumerate}
    \item related work: enough coverage, relevance to AAAI? citations from EMNLP, ACL, IJCAI or other venues are also ok 
    
    
   
\end{enumerate}

\section{List of things we will add if time permits/ window dressing}
\begin{enu}
    \item model name, model architecture diagram

\end{enu}

\section{List of experiments}
\begin{enumerate}
    \item baseline BERT models: general BERT, clinical BERT
    \item experiment to show the effect of data augmentation
    \item experiment to show the effect of scarcity of conflicting information: ratio of non-conflicting sample
    
    \item conducting error analysis for discussion and future work section
    \item experiment on reasoning?
    \item augmenting AMR-BERT with rules/ heuristics?
    
    
\end{enumerate}

==> sections/TDGL.tex <==
\begin{figure*}[!h]
\centering
  \includegraphics[scale=0.9]{Figures/AMR_Link_Example1.pdf}
  \caption{Our semantic representation for the health advice pair ('Consume alcohol in moderation', 'Do not drink alcoholic beverages.'). Visualized are the individual AMR graphs for Advice 1 and Advice 2 respectively, as well as the topic-linked version of the advice representation.}
\end{figure*}

\subsection{Topic-Driven Graph Linking}
The challenge with utilizing AMR graphs alongside pair-wise textual inputs is that the AMR graphs are only defined for contiguous pieces of text. The goal of Topic-Driven Graph Linking (TDGL), is to unify two disjoint graphs into a single semantic representation that accounts for the entire pairwise input. 

For a given pair of health advice $(W_1, W_2)$ we have two AMR graphs, $G_1 = (C_1, R_1)$ and $G_2 = (C_2, R_2)$, where $C$ denotes the set of semantic concepts and $R$ denotes the set of relations between semantic concepts. Furthermore, each graph has a set of alignments $A_1, A_2$ which represent a mapping between semantic concept nodes and input tokens  $A_i: W_i \rightarrow C_i$. In other words, AMR alignment data allows us to identify the exact input tokens responsible for producing the semantic concepts in the AMR graph. 


Recall that each pair of conflicting medical advice is annotated with a conflict topic $t$. The high-level goal of TDGL is to identify the token $w_i \in W_1$ and $w_j \in W_2$ that have the highest semantic similarity with our topic $t$. Using the alignment data, we can then construct a new relational triple ($c_i$, $:conflict$, $c_j$) that joins $G_1$ and $G_2$ thus creating a unified semantic representation. 
 
The result of TDGL is a new graph, $$G_3 = ([C_1 + C_2], [R_1 + R_2 + (c_i, :conflict, c_j)])$$

where $c_i \in C_1$ and $c_j \in C_2$ are the AMR concepts representing the medical conflict topic. We use $G_3$ as the AMR representation of our pair-wise model input. 
 %width=7.35in,height=2.54in
 
 
 \begin{table}
\begin{tabular}{llcccc}

\toprule
\textbf{Model} & F1 &  Precision &  Recall \\
\midrule
  RF + CRR    &  0.36/0.004 & 0.48/0.004 & 0.31/0.005 \\
  RF + CRC  &  0.10/0.005 &       0.15/0.04 &    0.10/0.004 \\
  RF + CRC + CRR &  0.32/.007 &       0.53/.004 &    0.24/.006 \\
  BERT  &  0.37/0.08 &       0.51/0.06 &    0.31/0.09 \\
  \hline
  BERT + CRR &  0.48/0.03 &       0.48/0.04 &    0.52/0.05 \\
  \ModelName  &  0.50/0.03 &       0.49/0.03 &    0.54/0.06\\
  \ModelName + CRR &   0.52/0.02  & 0.49/0.02 &    0.59/0.03 \\
\bottomrule
\end{tabular}
\caption{Mean/Standard Deviation over 5 runs of each experiment, each with a different random seed.} 
\label{results}
\end{table}

==> sections/oldIntro.tex <==

% medinfo and inconsistent med info: misinformation, conflicting information --> MCD

% why automatic MCD is important

% prior work and how our work is novel?

%  challenges of automatic MCD in the context of PLM

% our solution overview

% concrete list of contribution





As we continue to live through a global pandemic, now more than ever are people relying on online resources for medical advice \cite{Loomba2021}. In recent years, quick and easy access to health information has changed the way  people eat, exercise, and interact with medical professionals \cite{BujnowskaFedak2020}. A major limitation of online health platforms is their inability to provide contextually aware medical advice. That is to say, health advice provided online is most often without consideration of the end-users medical history. What if the user is advised to eat foods that interact poorly with their medications? What if the user is advised to perform vigorous exercise without knowledge of a pre-existing heart condition? Such questions  motivate the need for technology which automatically recognizes inconsistent health information across multiple relevant sources in effort to facilitate safer interactions with online health platforms. 

In this paper, we introduce the medical conflict detection (MCD) task. Given two pieces of health advice, the goal of MCD is to both identify the presence of a conflict \textit{and} to understand what type of conflict occurs. Note that understanding conflict type is crucial as we do not aim to resolve conflicts, but rather alert a user to a potential danger and aid them in their interpretation. For example, consider the  quantitative/temporal conflict in Table \ref{dataset}. This is a challenging multi-label conflict whose understanding is crucial to the user's health. To simply express that a conflict is present does not guide the user on how to react to the conflicting information on fiber consumption. Explicitly stating the conflict type communicates how one should be careful regarding \textit{how much } (quantitative) fiber one should eat as well as \textit{when } (temporal) fiber should be consumed.

%%%%%%
Conflicting medical information may arise for a number of reasons:  The information sources pertain to different health topics, one topic has conflicting underlying research, and more recently, we find that information sources may simply report false or conspiratory claims about a certain topic. The latter issue feels particularly relevant as the Covid-19 pandemic has also sparked an infodemic \cite{Buchanan2020}. Widespread medical disinformation is a danger to public health and extremely expensive to combat. In fact, in 2020 over \$471 million dollars were spent funding anti-misinformation campaigns worldwide \cite{cornish2020}. 


%%%%%%
Some prior work exists on MCD \cite{7917875, PREUM2017226} but no research explores the effectiveness of neural embedding models on this task. One of the main challenges with using models such as BERT \cite{bert} for MCD is that the task is inherently resource constrained. Furthermore, BERT is not built for multi-sentence inputs and often struggles with understanding long-range dependencies between words.  
To alleviate some of BERTs limitations, we propose the use of Abstract Meaning Representations (AMR) \cite{Banarescu2013AbstractMR}. We provide an example AMR graph in Figure \ref{amr_example} for reference. AMRs encode the relationships between all high-level concepts for a given text. This is useful for BERT as knowledge of semantic relations may help better understand long-range textual dependencies. Furthermore, AMRs encode positionless knowledge with respect to the input tokens, as they do not directly translate to English sentences. Given BERT's dependency on positional embeddings, it may be the case that AMRs can help alleviate this dependency. Evidence of BERT's need for external semantic information is shown in \cite{zhang2020semantics}, who utilize semantic role labels (SRL) to improve BERT's performance on pair-wise classification tasks such as Natural Language Inference. Given that AMRs are a richer semantic representation than SRL,  they have strong potential to aid BERT in downstream classification tasks. 

Additionally, AMRs contain information that is extremely relevant to conflict detection as they explicitly encode relations which are specific to the conflict types outlined in the dataset used in this work. For example, in Table \ref{dataset}, we predict conflict types such as direct, temporal, quantitative, and conditional, all of which have  relevant concepts and relations within the AMR vocabulary. We argue that state-of-the-art (SOTA) AMR parsers are able to extract high-level semantic information that is useful for detecting conflicts while alleviating some of BERT's limitations on resource constrained tasks. 

In this paper, our contributions are as follows:
\begin{itemize}
    \item We introduce the Medical Conflict Detection task in the context of neural language models. We provide a thorough investigation of the applicability of transformer-based embedding methods (i.e. BERT) for conflict identification. We further discuss limitations of BERT and propose an AMR-based solution to augment BERT for this task.
    \item We introduce a pair-wise AMR-based architecture that leverages pre-trained BERT models for Medical Conflict Detection. Our approach outperforms BERT by a 40\% increase in F1 score on average. To the best of our knowledge, this work is the first to successfully utilize non-gold label AMR graphs to increase the performance of a pair-wise classification task.
\end{itemize}


% some prior work on medical conflict detection, but no research on analyzing the effectiveness of neural embedding model for this task, i.e., how to adapt SOTA NLP models for such resource constrained, safety-critical NLP tasks. 
%%%%%



% [Comment: need to stress that we are not resolving any conflicts, we are trying to detect and identify them]







